On the automated verification of web applications with embedded SQL

A large number of web applications is based on a relational database together with a program, typically a script, that enables the user to interact with the database through embedded SQL queries and commands. In this paper, we introduce a method for formal automated verification of such systems which connects database theory to mainstream program analysis. We identify a fragment of SQL which captures the behavior of the queries in our case studies, is algorithmically decidable, and facilitates the construction of weakest preconditions. Thus, we can integrate the analysis of SQL queries into a program analysis tool chain. To this end, we implement a new decision procedure for the SQL fragment that we introduce. We demonstrate practical applicability of our results with three case studies, a web administrator, a simple firewall, and a conference management system.

==> app-invariants.tex <==

\section{Runnning Example: Invariants in FO\twoBD}\label{ap:invariants}
For simplicity we have written the invariants in Section~\ref{se:running} in first-order logic with counting quantifiers. 
Here we give equivalent formulas in FO\twoBD, i.e.\ without counting quantifiers and using only $x$ and $y$ to range over $\Dom$. 
Recall $\mathit{Inv}=\mathit{Inv}_1\land \mathit{Inv}_2$, where
\[
\begin{array}{lll}
\mathit{Inv}_1
&=& \forall_{\Domshort} x,y.\, \exists_{\Blshort}^{\leq 1} s.\, \exists_{\codesshort}^{\leq 1} c.\,\mathit{\nwlEmail}(x,y,s,c)
\\
\mathit{Inv}_2 &=& \forall_{\codesshort} c.\, (c\not=\mathit{nil}) \to \left(\exists^{\leq 1}_{\Domshort} x,y.\, \exists^{\leq 1}_{\Blshort} s.\, \mathit{\nwlEmail}(x,y,s,c)\right)
\end{array}
\]

$\mathit{Inv}_1$ is a shorthand for the following FO\twoBD\ sentence:
\[
 \forall_{\Domshort} x,y.\, \forall_{\Blshort} s_1,s_2.\, \forall_{\codesshort} c_1,c_2.\,\left(
 (s_1=s_2 \land c_1=c_2)\lor\bigvee_{i=1,2}\neg\mathit{\nwlEmail}(x,y,s_i,c_i)
 \right)
\]

For $\mathit{Inv}_2$ the same approach for eliminating counting quantifiers is not sufficient, since it requires four variables 
ranging over $\Dom$. Instead, $\mathit{Inv}_2$ is equivalent to 
\[
 \mathit{Inv}_{2,sub}\land \mathit{Inv}_{2,nwl}\land \mathit{Inv}_{2,user}
\]

$\mathit{Inv}_{2,sub}$ is 
\[
 \begin{array}{lll}
\forall_{\codesshort} c.\, (c\not=\mathit{nil}) \to 
\forall_{\Domshort} x,y.\, \left(\neg \mathit{\nwlEmail}(x,y,true,c) \lor
\neg\mathit{\nwlEmail}(x,y,false,c)\right)
\end{array}
\]
expressing that for every confirm code $c$, newsletter $n$ and user $u$, either $(n,u,true,c)$ or $(n,u,false,c)$ does not belong to $\nwlEmail$. 

$\mathit{Inv}_{2,nwl}$ is 
\[
 \begin{array}{lll}
\forall_{\codesshort} c.\, \forall_{\Domshort} x,y.\, (c\not=\mathit{nil} \land x\not=y) \to
\left(\forall_{\Blshort} s.\, \forall_{\Domshort} y.\, \neg \mathit{\nwlEmail}(x,y,s,c)\right) 
\lor \left(\forall_{\Blshort} s.\, \forall_{\Domshort} x.\, \neg\mathit{\nwlEmail}(y,x,s,c)\right)
\end{array}
\]
expressing that for every confirm code $c$, at most one newsletter $n$ belongs to a tuple of the form
$(n,u,s,c)$ in $\nwlEmail$. 

$\mathit{Inv}_{2,user}$ is
\[
 \begin{array}{lll}
\forall_{\codesshort} c.\, \forall_{\Domshort} x,y.\, (c\not=\mathit{nil} \land x\not=y) \to
\left(\forall_{\Blshort} s.\, \forall_{\Domshort} y.\, \neg \mathit{\nwlEmail}(y,x,s,c)\right) 
\lor \left(\forall_{\Blshort} s.\, \forall_{\Domshort} x.\, \neg\mathit{\nwlEmail}(x,y,s,c)\right)
\end{array}
\]
expressing that for every confirm code $c$, at most one user $u$ belongs to a tuple of the form
$(n,u,s,c)$ in $\nwlEmail$. 

Together these three sentences express that every confirm code belongs to at most a single row in $\nwlEmail$. 
Observe that the only variables ranging over $\Dom$ in $\mathit{Inv}_{2,sub}\land \mathit{Inv}_{2,nwl}\land \mathit{Inv}_{2,user}$
are $x$ and $y$. 



